Does Quality of Requirements Specifications matter? Combined Results of Two Empirical Studies

Background: Requirements Engineering is crucial for project success, and to this end, many measures for quality assurance of the software requirements specification (SRS) have been proposed. Goal: However, we still need an empirical understanding on the extent to which SRS are created and used in practice, as well as the degree to which the quality of an SRS matters to subsequent development activities. Method: We studied the relevance of SRS by relying on survey research and explored the impact of quality defects in SRS by relying on a controlled experiment. Results: Our results suggest that the relevance of SRS quality depends both on particular project characteristics and what is considered as a quality defect; for instance, the domain of safety critical systems seems to motivate for an intense usage of SRS as a means for communication whereas defects hampering the pragmatic quality do not seem to be as relevant as initially thought. Conclusion: Efficient and effective quality assurance measures must be specific for carefully characterized contexts and carefully select defect classes.

==> tbl_survey_corr_v1.tex <==
\begin{table*}[!t]
% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.3}

% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Impact of Project Parameters on the Relevance of the SRS (sig.~level $\alpha=0.05$)}
\label{tbl:survey_coef}
\centering
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{@{}p{3.0cm}rrrrlrrrlrrrlrrr@{}} \toprule
  \multicolumn{2}{c}{\multirow{3}{*}{\textbf{Parameter}}} 	& \multicolumn{7}{c}{\textbf{Impact on Documentation in SRS}} 																				& \phantom{a} &  \multicolumn{7}{c}{\textbf{Impact on Communication using SRS}} \\
	\multicolumn{2}{c}{}			 											&	\multicolumn{3}{c}{Completeness} 		& \phantom{a}	& \multicolumn{3}{c}{Level of Detail} 		& & \multicolumn{3}{c}{SRS used?} 	& \phantom{a}				& \multicolumn{3}{c}{SRS Ranking} \\ 
	\cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13} \cmidrule{15-17}
	\multicolumn{2}{c}{}														&	$\tau$~~ & $p$~~ & $p_{fdr}$~ && $\tau$~~ & $p$~~ & $p_{fdr}$~ && $\tau$~~ & $p$~~ & $p_{fdr}$~ && $\tau$~~ & $p$~~ & $p_{fdr}$~ \\ \midrule

\multirow{2}{*}{\formatpar{Team Size}}				& Proj.\ 					& -0.03 & 0.84 & 1.00 	&& -0.21 & 0.22 & 0.72 		&& 0.22 & 0.22 & 0.60 		&& 0.17 & 0.41 & 0.65  \\
																							& Gen.\ 					& -0.04 & 0.80 & 0.87 	&& -0.04 & 0.81 & 0.89		&& 0.14 & 0.45 & 0.79 		&& -0.07& 0.73 & 0.93  \\ \addlinespace
																			
\multirow{2}{*}{\formatpar{Team Distribution}}		& Proj.\ 			& 0.00 & 1.00 & 1.00 		&& -0.14 & 0.41 & 0.72 		&& 0.05 & 0.76 & 0.90 		&& -0.01 & 0.97 & 0.97  \\
																							& Gen.\ 					& -0.07 & 0.68 & 0.86 	&& 0.06 & 0.70 & 0.89 		&& -0.13 & 0.47 & 0.79 		&& -0.06 & 0.76 & 0.93  \\ \addlinespace
																																						 
\multirow{2}{*}{\formatpar{Team Turnover}}		& Proj.\ 					& 0.00 & 1.00 & 1.00 		&& -0.11 & 0.52 & 0.72 		&& -0.03 & 0.88 & 0.90 		&& \cellmod 0.30 & 0.14 & 0.39 \\
																							& Gen.\ 					& 0.03 & 0.87 & 0.87 		&& -0.04 & 0.79 & 0.89 		&& 0.11 & 0.54 & 0.79 		&& 0.29 & 0.16 & 0.79  \\ \addlinespace

\multirow{2}{*}{\formatpar{Management unavailable}}		& Proj.\ 	& -0.01 & 0.96 & 1.00 	&& 0.09 & 0.60 & 0.73 		&& 0.08 & 0.66 & 0.90 		&& 0.24 & 0.25 & 0.55  \\
																							& Gen.\ 					& 0.07 & 0.70 & 0.86 		&& \cellmod 0.43 & 0.01 & 0.07 		&& 0.17 & 0.35 & 0.79 		&& \cellmod 0.39 & 0.06 & 0.66  \\ \addlinespace
																			
\multirow{2}{*}{\formatpar{Financial controlling req.}}		& Proj.\ & 0.02 & 0.93 & 1.00 && -0.06 & 0.71 & 0.78 		&& 0.05 & 0.78 & 0.90 		&& 0.13 & 0.54 & 0.74  \\
																							& Gen.\ 					& -0.14 & 0.38 & 0.84		&& -0.02 & 0.89 & 0.89 		&& 0.22 & 0.20 & 0.79			&& -0.18 & 0.36 & 0.79  \\ \addlinespace
																			
\multirow{2}{*}{\formatpar{Measurements req.}}		& Proj.\ 			& 0.28 & 0.10 & 0.37 		&& 0.27 & 0.11 & 0.72 		&& -0.02 & 0.90 & 0.90 		&& \cellmod 0.36 & 0.08 & 0.31  \\
																							& Gen.\ 					& \cellmod 0.30 & 0.07 & 0.20 		&& \cellmod 0.51 & 0.00 & 0.02 		&& 0.09 & 0.61 & 0.79 		&& -0.21 & 0.31 & 0.79 \\ \addlinespace
																			
\multirow{2}{*}{\formatpar{Many stakeholders}}		& Proj.\ 			& -0.10 & 0.57 & 1.00 	&& 0.04 & 0.83 & 0.83 		&& -0.03 & 0.85 & 0.90 		&& -0.01 & 0.97 & 0.97  \\
																							& Gen.\ 					& -0.11 & 0.52 & 0.86		&& 0.20 & 0.23 & 0.64 		&& 0.10 & 0.58 & 0.79 		&& -0.02 & 0.94 & 0.94 \\ \addlinespace
																																						 
\multirow{2}{*}{\formatpar{Stakeholder unavailable}}		& Proj.\ 	& -0.17 & 0.33 & 0.72 && 0.11 & 0.53 & 0.72 		&& 0.17 & 0.35 & 0.77 		&& 0.17 & 0.41 & 0.65  \\
																							& Gen.\ 					& -0.09 & 0.60 & 0.86		&& \cellmod 0.30 & 0.08 & 0.29 		&& 0.07 & 0.69 & 0.79 		&& 0.11 & 0.58 & 0.93   \\ \addlinespace

\multirow{2}{*}{\formatpar{High Complexity}}		& Proj.\ 				& \cellmod -0.34 & \cellmod 0.05 & 0.28 	&& -0.13 & 0.47 & 0.72 		&& -0.23 & 0.21 & 0.60 		&& -0.09 & 0.66 & 0.81  \\
																							& Gen.\ 					& \cellmod -0.32 & 0.06 & 0.20 	&& -0.07 & 0.66 & 0.89 		&& 0.12 & 0.51 & 0.79 		&& 0.03 & 0.87 & 0.94 \\ \addlinespace
																			
\multirow{2}{*}{\formatpar{Safety/Security relevant}}		& Proj.\ 	& \cellmod 0.46 & \cellmod 0.01 & 0.08 	&& 0.16 & 0.35 & 0.72 		&& 0.24 & 0.19 & 0.60 		&& \cellmod0.49 & \cellmod 0.02 & 0.21  \\
																							& Gen.\ 					& \cellmod 0.38 & \cellmod 0.02 & 0.11 		&& 0.12 & 0.48 & 0.87 		&& 0.06 & 0.74 & 0.79 		&& 0.25 & 0.23 & 0.79 \\ \addlinespace
																			
\textbf{Release cycle}		& Proj.\ 					& -0.24 & 0.15 & 0.41 	&& -0.25 & 0.14 & 0.72 		&& 0.23 & 0.19 & 0.60 		&& \cellmod0.35 & 0.08 & 0.31 \\ \addlinespace																																			
\midrule
																			
\multirow{2}{*}{\formatpar{Previous cooperation}}		& Proj.\ 		& -0.10 & 0.57 & 0.57 	&& -0.21 & 0.22 & 0.43 		&& -0.20 & 0.27 & 0.95 		&& -0.09 & 0.67 & 0.79  \\
																							& Gen.\ 					& -0.06 & 0.72 & 0.95		&& 0.01 & 0.96 & 0.96 		&& -0.03 & 0.86 & 0.86  	&& -0.20 & 0.34 & 0.67 \\ \addlinespace
																			
\multirow{2}{*}{\formatpar{Good cooperation}}		& Proj.\ 				& \cellmod 0.41 & \cellmod 0.02 & 0.09 		&& 0.23 & 0.20 & 0.43 		&& 0.01 & 0.95 & 0.95 		&& -0.16 & 0.49 & 0.79  \\
																							& Gen.\ 					& 0.25 & 0.15 & 0.29 		&& 0.01 & 0.96 & 0.96 		&& -0.20 & 0.29 & 0.77 		&& -0.25 & 0.23 & 0.67  \\ \addlinespace
																			
\multirow{2}{*}{\formatpar{Small Budget}}		& Proj.\ 						& 0.11 & 0.53 & 0.57 		&& -0.03 & 0.87 & 0.87 		&& -0.06 & 0.74 & 0.95 		&& -0.06 & 0.79 & 0.79 \\
																							& Gen.\ 					& -0.01 & 0.95 & 0.95 	&& -0.14 & 0.38 & 0.87 		&& 0.15 & 0.38 & 0.77 		&& 0.04 & 0.85 & 0.85  \\ \addlinespace
																																						 
\multirow{2}{*}{\formatpar{Volatile Requirements}}		& Proj.\ 	& -0.20 & 0.25 & 0.50 	&& -0.08 & 0.63 & 0.84 		&& -0.12 & 0.50 & 0.95 		&& -0.06 & 0.79 & 0.79  \\
																							& Gen.\ 					& \cellmod -0.49 & \cellmod 0.00 & \cellmod 0.01 	&& -0.13 & 0.43 & 0.87 		&& -0.05 & 0.79 & 0.86		&& -0.07 & 0.73 & 0.85  \\ \addlinespace
																			
\midrule

\textbf{Prev.~Domain Knowledge}		& Proj.\ 					& - & - & - 								&& 		- & - & - 							&& 0.29 & 0.11 & 0.23 	&& 0.07 & 0.75 & 0.91  \\ \addlinespace
																			
\textbf{Prev.~Product Knowledge}		& Proj.\ 					& - & - & - 								&&    - & - & - 		&& -0.09 & 0.63 & 0.63 		&& 0.02 & 0.91 & 0.91 \\

\bottomrule											
\end{tabular}
\end{table*}

==> tbl_survey_corr_v2.tex <==
\begin{table*}[!t]
% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.3}

% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Impact of Project Parameters on the Relevance of the SRS (sig.~level $\alpha=0.05$)}
\label{tbl:survey_coef}
\centering
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{@{}p{3.0cm}rrrrlrrrlrrrlrrr@{}} \toprule
  \multicolumn{2}{c}{\multirow{3}{*}{\textbf{Parameter}}} 	& \multicolumn{7}{c}{\textbf{Impact on Documentation in SRS}} 																				& \phantom{a} &  \multicolumn{7}{c}{\textbf{Impact on Communication using SRS}} \\
	\multicolumn{2}{c}{}			 											&	\multicolumn{3}{c}{Completeness} 		& \phantom{a}	& \multicolumn{3}{c}{Level of Detail} 		& & \multicolumn{3}{c}{SRS used?} 	& \phantom{a}				& \multicolumn{3}{c}{SRS Ranking} \\ 
	\cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13} \cmidrule{15-17}
	\multicolumn{2}{c}{}														&	$\tau$~~ & $p$~~ & $p_{fdr}$~ && $\tau$~~ & $p$~~ & $p_{fdr}$~ && $\tau$~~ & $p$~~ & $p_{fdr}$~ && $\tau$~~ & $p$~~ & $p_{fdr}$~ \\ \midrule

%% START --- GENERATED AUTOMATICALLY (R)


\multirow{2}{*}{\formatpar{Team Size}} & Proj.\ &-0.08 & 0.63 & 0.85 && 0.06 & 0.69 & 0.94 && 0.07 & 0.65 & 0.8 && 0.2 & 0.28 & 0.63 \\
& Gen.\ & -0.08 & 0.6 & 0.82 && 0.18 & 0.26 & 0.47 && 0.04 & 0.81 & 1 && 0.05 & 0.79 & 0.89 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Team Distribution}} & Proj.\ &0.06 & 0.7 & 0.85 && 0.03 & 0.87 & 0.94 && 0.09 & 0.59 & 0.8 && 0.02 & 0.92 & 0.92 \\
& Gen.\ & -0.04 & 0.81 & 0.84 && 0.25 & 0.12 & 0.32 && -0.14 & 0.41 & 1 && 0.09 & 0.62 & 0.85 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Team Turnover}} & Proj.\ &-0.02 & 0.88 & 0.93 && 0.05 & 0.75 & 0.94 && -0.01 & 0.94 & 0.94 && 0.22 & 0.26 & 0.63 \\
& Gen.\ & -0.09 & 0.56 & 0.82 && 0.01 & 0.97 & 1 && -0.04 & 0.83 & 1 && 0.19 & 0.32 & 0.75 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Management unavailable}} & Proj.\ &0.01 & 0.93 & 0.93 && 0.06 & 0.72 & 0.94 && 0.1 & 0.54 & 0.8 && 0.13 & 0.52 & 0.73 \\
& Gen.\ & 0.03 & 0.84 & 0.84 && 0.29 & 0.07 & 0.26 && 0.08 & 0.61 & 1 && 0.26 & 0.19 & 0.75 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Financial controlling req.}} & Proj.\ &0.09 & 0.59 & 0.85 && 0.13 & 0.41 & 0.94 && 0.15 & 0.37 & 0.77 && 0.12 & 0.53 & 0.73 \\
& Gen.\ & -0.05 & 0.73 & 0.84 && 0.1 & 0.51 & 0.7 && 0.3 & 0.07 & 0.71 && -0.18 & 0.34 & 0.75 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Measurement req.}} & Proj.\ &\cellmod 0.34 & \cellmod 0.03 & 0.18 && 0.28 & 0.08 & 0.46 && 0.14 & 0.4 & 0.77 && 0.27 & 0.17 & 0.62 \\
& Gen.\ & \cellmod 0.37 & \cellmod 0.02 & 0.08 && \cellmod 0.37 & \cellmod 0.02 & 0.16 && 0.25 & 0.13 & 0.71 && -0.21 & 0.29 & 0.75 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Many stakeholders}} & Proj.\ &-0.1 & 0.55 & 0.85 && 0.06 & 0.73 & 0.94 && -0.05 & 0.77 & 0.85 && 0.04 & 0.84 & 0.92 \\
& Gen.\ & -0.11 & 0.51 & 0.82 && 0.17 & 0.3 & 0.47 && 0.14 & 0.42 & 1 && -0.15 & 0.46 & 0.8 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Stakeholder unavailable}} & Proj.\ &-0.12 & 0.46 & 0.85 && 0.02 & 0.92 & 0.94 && 0.21 & 0.22 & 0.77 && 0.08 & 0.69 & 0.84 \\
& Gen.\ & -0.17 & 0.29 & 0.64 && 0.18 & 0.27 & 0.47 && 0 & 1 & 1 && -0.03 & 0.89 & 0.89 \\ \addlinespace 

\multirow{2}{*}{\formatpar{High complexity}} & Proj.\ &\cellmod -0.31 & 0.06 & 0.21 && 0.02 & 0.92 & 0.94 && -0.18 & 0.31 & 0.77 && -0.12 & 0.53 & 0.73 \\
& Gen.\ & \cellmod -0.36 & \cellmod 0.02 & 0.08 && 0.03 & 0.87 & 1 && 0.03 & 0.86 & 1 && 0.03 & 0.89 & 0.89 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Safety/Security relevant}} & Proj.\ &\cellmod 0.38 & \cellmod 0.02 & 0.18 && \cellmod 0.36 & \cellmod 0.03 & 0.29 && 0.14 & 0.42 & 0.77 && \cellmod 0.52 & \cellmod 0.01 & 0.08 \\
& Gen.\ & \cellmod 0.32 & \cellmod 0.04 & 0.12 && \cellmod 0.34 & \cellmod 0.03 & 0.16 && 0.01 & 0.96 & 1 && \cellmod 0.38 & \cellmod 0.05 & 0.51 \\ \addlinespace 

\multirow{1}{*}{\formatpar{Release Cycle Length}} & Proj.\ &-0.19 & 0.24 & 0.67 && -0.01 & 0.94 & 0.94 && 0.26 & 0.11 & 0.77 && \cellmod 0.33 & 0.08 & 0.46 \\
\addlinespace

 \midrule 

\multirow{2}{*}{\formatpar{Previous cooperation}} & Proj.\ &-0.03 & 0.83 & 0.83 && \cellmod -0.32 & \cellmod 0.04 & 0.17 && -0.11 & 0.52 & 0.81 && -0.07 & 0.71 & 0.81 \\
& Gen.\ & -0.01 & 0.95 & 0.95 && -0.18 & 0.25 & 0.44 && 0.03 & 0.87 & 0.96 && -0.17 & 0.38 & 0.81 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Good cooperation}} & Proj.\ &\cellmod 0.44 & \cellmod 0.01 & \cellmod 0.04 && 0.2 & 0.23 & 0.31 && 0.07 & 0.71 & 0.81 && -0.05 & 0.81 & 0.81 \\
& Gen.\ & 0.26 & 0.11 & 0.23 && -0.16 & 0.33 & 0.44 && -0.07 & 0.69 & 0.96 && -0.29 & 0.15 & 0.81 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Small Budget}} & Proj.\ &0.12 & 0.45 & 0.6 && -0.2 & 0.21 & 0.31 && 0.04 & 0.81 & 0.81 && -0.14 & 0.48 & 0.81 \\
& Gen.\ & 0.01 & 0.95 & 0.95 && -0.28 & 0.07 & 0.28 && 0.18 & 0.28 & 0.96 && 0.02 & 0.92 & 0.81 \\ \addlinespace 

\multirow{2}{*}{\formatpar{Volatile Requirements}} & Proj.\ &-0.21 & 0.19 & 0.38 && -0.05 & 0.76 & 0.76 && -0.08 & 0.62 & 0.81 && -0.1 & 0.59 & 0.81 \\
& Gen.\ & \cellmod -0.47 & \cellmod 0 & \cellmod 0.01 && 0 & 1 & 1 && -0.01 & 0.96 & 0.96 && -0.13 & 0.51 & 0.81 \\ \addlinespace 


 \midrule 

\multirow{1}{*}{\formatpar{Prev. Domain Knowledge}} & Proj.\ &- & - & - && - & - & - && 0.28 & 0.09 & 0.18 && 0 & 1 & 1 \\ \addlinespace
\multirow{1}{*}{\formatpar{Prev. Product Knowledge}} & Proj.\ &- & - & - && - & - & - && -0.03 & 0.85 & 0.85 && -0.08 & 0.68 & 1 \\ \addlinespace


%% END --- GENERATED AUTOMATICALLY (R)

\bottomrule											
\end{tabular}
\end{table*}
